PERLE: Powerful Energy Recovery Linac for Experiments - Conceptual Design Report

A conceptual design is presented of a novel ERL facility for the development and application of the energy recovery technique to linear electron accelerators in the multi-turn, large current and large energy regime. The main characteristics of the powerful energy recovery linac experiment facility (PERLE) are derived from the design of the Large Hadron electron Collider, an electron beam upgrade under study for the LHC, for which it would be the key demonstrator. PERLE is thus projected as a facility to investigate efficient, high current (> 10 mA) ERL operation with three re-circulation passages through newly designed SCRF cavities, at 801.58 MHz frequency, and following deceleration over another three re-circulations. In its fully equipped configuration, PERLE provides an electron beam of approximately 1 GeV energy. A physics programme possibly associated with PERLE is sketched, consisting of high precision elastic electron-proton scattering experiments, as well as photo-nuclear reactions of unprecedented intensities with up to 30 MeV photon beam energy as may be obtained using Fabry-Perot cavities. The facility has further applications as a general technology test bed that can investigate and validate novel superconducting magnets (beam induced quench tests) and superconducting RF structures (structure tests with high current beams, beam loading and transients). Besides a chapter on operation aspects, the report contains detailed considerations on the choices for the SCRF structure, optics and lattice design, solutions for arc magnets, source and injector and on further essential components. A suitable configuration derived from the here presented design concept may next be moved forward to a technical design and possibly be built by an international collaboration which is being established.

==> Instructions.tex <==
\markboth{Instructions} {right head}
\chapter*{Instructions}
\markboth{Instructions}{right head}\markright{Instructions}


Contributions can be prepared in \LaTeX\  using this template.\\
Please prepare your manuscript according to these instructions. 
 {\em Do not change} the {\em main.tex} file provided.\\

{\bf{In case of any questions or problems, please send an email to Alessandra Valloni }
(alessandra.valloni@cern.ch).}

\section*{Typesetting a document using \LaTeX}

To make things simple you need just to open the file {\em yoursection}.tex and typeset your
contribution.  Then run the main file {\em main.tex} to generate the pdf file which will help
you to have an idea of what your contribution will look like.
You don't need to add packages or include any additional styleset.
Please open your page and type your contribution.

\subsection*{Figures}
\label{sec:figures}

Figure \ref{Fig:Example} shows an example of a figure and related
caption.  Please ensure that all symbols and lettering in your figures
are large enough.  You may insert colour figures, but it is your
responsibility to check that they print correctly in black and white.
You may submit an additional black and white version.

\begin{figure}[H]
%\centerline{\includegraphics[clip=,width=0.35\textwidth]{LogoLHeC
%}}
 \centering
  \includegraphics[width=0.55\textwidth]{LogoLHeC.jpg}
\caption{Example figure with example caption.}\label{Fig:Example}
\end{figure}

Captions of figures and tables appear {\em below} the figure/table.
When referring to Figure~\ref{Fig:Example} capitalise the first letter
and use the latex `\verb?\ref?' command to make references to your
figures.

\subsection*{Mathematics}
It is recommended to avoid the numbering of equations when not
necessary. When dealing with equation arrays, it could be
necessary to label several (in)equalities. You can do it using the
'\verb?\stackrel?' operator; example:

\begin{eqnarray}
c&=&|d|+|e|\nonumber\\
&\stackrel{\text{(a)}}{=}&d+e\nonumber\\
&\stackrel{\text{(b)}}{\geq}&\sqrt{f}\enspace,
\end{eqnarray}
\noindent where the equality (a) results from the fact that both
$d$ and $e$ are positive while (b) comes from the definition of
$f$.


\subsection*{Bibliography}

Please use the bibtex information as given by SPIRES to make
citations.
Simply create a bibtex file {\em (yoursection.bib)} and then add your bibtex
information from SPIRES to that file.\\
{\bf Example}\\
LHeC CDR \cite{Abelleira2012}. Look at the file {\em bib.bib} to see how the citation has been exported.

Please use as cite key first author's surname and year (Abelleira2012) and add the reference in 
{\em yoursection}.bib.



When your work is done please send two files {\em yoursection}.tex and  {\em yoursection}.bib
to {\bf
\color{red}
alessandra.valloni@cern.ch 
\color{black}
and
\color{blue}
max.klein@desy.de}



==> RFdevelopmentswithbeam.tex <==
\subsection{Frequency variation for cavity tests}
%
PERLE is described below 
in a default configuration including cavities at 
801.58 MHz in up to 4 cryomodules and a bunch spacing of 25 ns. 
To gain flexibility and potential as a test facility to test cavities and cryomodules 
with beam, PERLE can however also be configured for use at a number of frequencies commonly used in accelerator facilities world-wide, in particular at 352 MHz (Linac4, ESS), 401 MHz 
(LHC, FCC), 704 MHz (ESS), 802 MHz (LHC, FCC and LHeC) and 1300 MHz (ILC, XFEL, \dots).  
To make this possible, the injector must be based on a photocathode with a laser pulser that can
 be operated at $f_0$ = 12.146 MHz and a buncher/booster system that equally operates at a harmonic of $f_0$. 
The frequency of 12.146 MHz was of course chosen on purpose as a common subharmonic 
of these commonly used frequencies, the exact harmonic frequencies accessible as PERLE 
main RF are given in Table~\ref{RF_ranges}. assuming the possibility to tune the subharmonic 
$f_0$ by moderate $\pm $ 4 kHz. 
This assumption translates to a tuning range at 801 MHz of $\pm $ 264 kHz, 
which should be implemented in the buncher/booster.

\begin{table}
\begin{center}
\begin{tabular}{cccccc}
\hline
h & 29&33&58&66&107\\
\hline
$h(f_0 - 4 kHz)$ & 352.118 MHz & 400.686 &704.236 MHz& 801.372 MHz & 1299.19 MHz\\
$h(f_0 + 4 kHz)$ & 352.350 MHz & 400.950 &704.700 MHz& 801.900 MHz & 1300.05 MHz\\
\hline
\end{tabular}
\caption{Main RF ranges for selected harmonics accessible to PERLE with an injector pulsed at $f_0$ =12.146 MHz. It allows RF developments at most commonly used frequencies.}\label{RF_ranges}
\end{center}
\end{table}


Referring to the description of source and injector in ~\ref{sec:sourceandinjector}, 
it is clear that a bunch repetition frequency of 40.1 MHz (25 ns) is not compatible 
with most of the above frequencies and should be adapted to either 12.146 MHz, 
where it could be used with all mentioned frequencies with the caveat that larger 
bunch charge would have to be generated for a similar average current (challenging 1 nC for 12 mA!). 
For tests at 401 MHz and 802 MHz however, a bunch repetition frequency of 36.438 MHz can be chosen, 
which would be close enough to the LHeC parameters to be relevant. 
It would produce 12 mA of beam current with 329 pC bunch charge. 
The filling scheme and bunch recombination pattern (Figures ~\ref{FIG_REC_PATTERN_1}, ~\ref{FIG_REC_PATTERN_2}) 
would have to be adapted  \textit{mutatis mutandis} (harmonic 20 would now become harmonic 22) with individual bunch spacings 7$\lambda$-8$\lambda$-7$\lambda$. 
The buncher/booster system described in ~\ref{sec:sourceandinjector} 
can remain unchanged. It is noteworthy that for 
a bunch repetition frequency of 12.146 MHz, captured and 
accelerated in this booster at 801 MHz, the frequency of the cavities in the ERL 
might still be 704 MHz and 1300 MHz. Even the simultaneous 
operation at different frequencies in the same linac is not excluded.

